From Search To Sampling: Generative Models For Robust Algorithmic Recourse

Algorithmic Recourse provides recommendations to individuals who are adversely impacted by automated model decisions, on how to alter their profiles to achieve a favorable outcome. Effective recourse methods must balance three conflicting goals: proximity to the original profile to minimize cost, plausibility for realistic recourse, and validity to ensure the desired outcome. We show that existing methods train for these objectives separately and then search for recourse through a joint optimization over the recourse goals during inference, leading to poor recourse recommendations. We introduce GenRe, a generative recourse model designed to train the three recourse objectives jointly. Training such generative models is non-trivial due to lack of direct recourse supervision. We propose efficient ways to synthesize such supervision and further show that GenRe's training leads to a consistent estimator. Unlike most prior methods, that employ non-robust gradient descent based search during inference, GenRe simply performs a forward sampling over the generative model to produce minimum cost recourse, leading to superior performance across multiple metrics. We also demonstrate GenRe provides the best trade-off between cost, plausibility and validity, compared to state-of-art baselines. Our code is available at: https://github.com/prateekgargx/genre.

==> existing.tex <==


\section{Existing Approaches and their Limitations}
Before introducing our solution, we first highlight the failure modes of commonly used recourse methods, underscoring the need for improved models. We categorize prior methods into three main families:
\textcolor{blue}{Limitations of existing approaches
\begin{itemize}
    \item Joint of loss on classifier and cost could land either be too close to the boundary (need figure) or on spurious boundaries (Current Figure 1)
    \item Existing method of biasing selection to be on data manifold have practical difficulties --- for example choosing the optimal $\lambda$ (ToDo --- optimal $\lambda$ is different for different datasets, and small lambda gives high recouse cost, large lambda again on boundary)
\end{itemize}
\todo[inline]{L: How abt these sub-headings}
\begin{itemize}[leftmargin=10pt] 
    \item Methods that heavily depend on the classifier $h$. 
    \item Adversarially robust methods that aim to provide resilient recourse. 
    \item Methods focused on generating in-domain counterfactuals. 
\end{itemize}
}

% $\xcf = \arg\min_{\vx'} \text{cost}(\vx, \vx') \text{ s.t. } h(\vx') = \desiredlbl$


% Conventionally, recourse is expressed as the optimization problem:
% \begin{align}
% \xcf &= \arg\min_{\xcf \in \mathcal{A}} \ell(\proxycls(\vx'), \desiredlbl) + \lambda C(\vx, \vx')  \label{eq:vanilla_rec}
% \end{align}

% where $\ell$ is the cross-entropy loss, and $\mathcal{A}$ denotes the actionable search space of counterfactuals for $\vx$. For instance, $\mathcal{A}$ prevents changes to immutable features such as gender, etc. Finally, $\lambda > 0$ is a weight that trades-off cost with the log likelihood on the desired label. While classifier $h$ closely approximates the decisions made by $\goldcls$ within the training domain, its behavior becomes unpredictable and may significantly diverge from $\goldcls$ on out-of-domain instances.
% \todo[inline]{PG:need to write this more nicely}
% Such a behavior is commonly explained using the Roshomon Effect. Intuitively, for a given training dataset $\trnD$ and a loss $\epsilon > 0$, many models can achieve a training loss less than or equal to $\epsilon$. However, some of these models may exhibit a substantial increase in loss when applied to instances that deviate from the training distribution. In the next section, show examples for such failure modes. 

We analyze the failure modes of prior methods using three 2D toy datasets: \texttt{moons}, \texttt{circles} from \texttt{sklearn}, and \texttt{corr}. Further details on these datasets are provided in Appendix \ref{app:syntheticdata}. For all methods, we use their publicly available implementations from CARLA (\cite{pawelczyk2021carla}) with default hyperparameters. The classifier $h$ is trained using a MLP with ReLU activations (details in Appendix \ref{app:hyperparams}). In Fig. \ref{fig:truevsAnn}, we illustrate the boundaries of both $h$ and $\goldcls$. We draw specific attention to $h$ learned on the \texttt{corr} dataset, where we can see a spurious decision boundary towards the lower-left. \todo{L: @P, Pls zoom-in Fig. 1 to show the spurious bdry} 

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{images/true_vs_ann_boundary.png}
    \caption{Top Row: True Classifier Boundary; Bottom Row: Learned Classifier Boundary using a ReLU Network. \todo[inline]{P:replace top row with analytic boundary: even better, superimpose with ann boundary -- how?}}
    \label{fig:truevsAnn}
\end{figure}

\xhdr{Many methods map instances very close to boundary} 

The representative methods that fall into this category are: 
\texttt{Wachter}(\cite{wachter2017counterfactual}), \texttt{GS}(\cite{laugel2017inverseGS}), and \texttt{DICE}(\cite{mothilal2020dice}). These algorithms find recourse by solving a variant of the following objective: $\arg\min_{\xcf \in \mathcal{A}(\vx); \proxycls(\xcf)\geq 0.5} C(\vx, \vx')$. As noted by \cite{fokkema2024risks}, such methods often push instances near the boundary of $h$, as we can see for \texttt{Wachter} in \ref{fig:wacht_fails}. We provide results for \texttt{DICE} and \texttt{GS}
in Appendix \ref{app:additionalexp}. We make the following observations:

\begin{enumerate}[leftmargin=10pt]
    \item Firstly, finite-sample training of $h$ can distort its decision boundary away from that of the true $P(Y|X)$. Furthermore, even if $h$ were to be assumed as the final decision-making entity, recourse instances found by these methods have an equal probability of being assigned both the labels. 
    \item As seen with the \texttt{corr} dataset, $h$ can sometimes develop spurious boundaries out-of-distribution, leading these algorithms to predict recourse near them. Such recourse outputs are not {\em realistic}, and are therefore prone to be invalidated during inference.
\end{enumerate}

\todo[inline]{P: Can we claim that any trained classifier is most uncertain at the boundary?}
Next we see methods which attempt to shield from over-reliance on the classifier by mapping recourse at some `margin' away from the boundary.

\xhdr{Methods which map instances away from the boundary}

The representative methods that predict recourse that remain valid under small changes to the classifier $h$ on which they are learned are: \texttt{ROAR}(\cite{upadhyay2021ROAR}), \texttt{PROBE}(\cite{pawelczyk2022PROBE}). \texttt{ROAR} aims to achieve robustness by optimizing recourse for worst-case but bounded model shifts. \texttt{PROBE}, in contrast, finds recourse at points where $h$ consistently assigns the desired label to all points within an $\epsilon$-ball around it.
% 
% \texttt{ROAR}(\cite{upadhyay2021ROAR}) is a method which optimises for recourse under worst case model shift. Recourse can still get invalidated if the user implementation of recourse is noisy. \texttt{PROBE}(\cite{pawelczyk2022PROBE}) is method which allows users to specify a invalidation rate under gaussian noise to address the issue.
% 
Both these methods end up with an objective that pushes recourse instances away from the boundary. We also note that both methods were originally designed for linear models and later extended to non-linear models using local linear approximations such as \texttt{LIME} (\cite{ribeiro2016lime}). We make the following observations from Fig. \ref{fig:all_recourse_fails}: 
\begin{enumerate}[leftmargin=10pt]
   \item \texttt{ROAR} fails to generate valid recourse outputs for \texttt{corr} and \texttt{circles}. For \texttt{circles}, this issue likely stems from the difficulty in approximating the highly non-linear decision boundary using local linear approximations. In the \texttt{moons} dataset, \texttt{ROAR} incurs significantly higher costs and ventures out of distribution. Further, we found this method to be highly sensitive to the choice of hyperparameters.
    \todo[inline]{P: it is not clear why this failed in corr}
    \item \texttt{PROBE}'s reliance on $h$ makes it encounter challenges in \texttt{corr} because of the spurious decision boundary, similar to the \texttt{wachter} method. On \texttt{circles}, it achieves a very high cost. The main reason is in its pursuit to push the recourse $\vx'$ away from the decision boundary near $\vx$, it often ends up landing at another boundary away from $\vx$; while incurring huge costs. For the \texttt{moons} dataset, the method struggles with the highly non-linear nature of the classifier, frequently failing to produce valid recourse for most instances.
    \todo[inline]{P: Only difference between \texttt{ROAR} and \texttt{PROBE} on this dataset that PROBE won the hyperparam lottery} 
\end{enumerate}


\xhdr{Methods which generate likely counterfactuals.} These methods employ generative models to ensure that the recourse predicted during inference remains close to the training data manifold on which the models are trained. \texttt{REVISE} (\cite{joshi2019revise}) \texttt{CRUDS}(\cite{downs2020cruds}) uses variants of VAE(\cite{kingma2013auto}) to ensure that the generated recourse instances are near the data manifold, and  performs gradient descent in latent space to optimize the recourse instance. \texttt{CCHVAE} (\cite{pawelczyk2020cchvae}) uses random search in latent space and filters out instances that correctly flip the predictions.  We show the result of \texttt{CRUDS} in \ref{fig:cchvae_fails}. 

% Even though, \texttt{CCHVAE} improves on all the above mentioned problems, we notice that 1.) every input is assigned the same recourse output. 2.) Recourse instances do not lie on the data manifold. 

\todo[inline]{write why vae fails to capture this distribution}
\begin{figure}[H]
    \centering
    \begin{subfigure}[b]{1\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/wachter.png}
        \caption{\texttt{Wachter}(\cite{wachter2017counterfactual})}
        \label{fig:wacht_fails}
    \end{subfigure}

    \begin{subfigure}[b]{1\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/ROAR.png}
        \caption{\texttt{ROAR}(\cite{upadhyay2021ROAR})}
        \label{fig:roar_fails}
    \end{subfigure}


% \end{figure}
% \begin{figure}[ht]\ContinuedFloat
    \begin{subfigure}[b]{1\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/PROBE.png}
        \caption{\texttt{PROBE}(\cite{pawelczyk2022PROBE})}
        \label{fig:probe_fails}
    \end{subfigure}
    
    \begin{subfigure}[b]{1\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/cchvae.png}
        \caption{\texttt{CCHVAE}(\cite{pawelczyk2020cchvae})}
        \label{fig:cchvae_fails}
    \end{subfigure}
    
g    \caption{Comparison of different recourse methods}
    \label{fig:all_recourse_fails}
\end{figure}


